A Survey of Autonomous Driving: Common Practices and Emerging Technologies

Automated driving systems (ADSs) promise a safe, comfortable and efficient driving experience. However, fatalities involving vehicles equipped with ADSs are on the rise. The full potential of ADSs cannot be realized unless the robustness of state-of-the-art improved further. This paper discusses unsolved problems and surveys the technical aspect of automated driving. Studies regarding present challenges, high-level system architectures, emerging methodologies and core functions: localization, mapping, perception, planning, and human machine interface, were thoroughly reviewed. Furthermore, the state-of-the-art was implemented on our own platform and various algorithms were compared in a real-world driving setting. The paper concludes with an overview of available datasets and tools for ADS development.

==> Makefile <==
PLT=pdflatex -draftmode
PDFPLT=pdflatex
BTX=bibtex
XDV=xdvi-ja.real 
DPDF=dvipdfmx
DPS=dvips -Ppdf -R0 -ta4
PS2PDF=ps2pdf -dCompatibilityLevel=1.4 -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=a4
GV=gv
AC=evince
EMCS=emacs
#GS=gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dNOPAUSE -dQUIET -dBATCH -sOutputFile=$(T)-compressed.pdf 
GS=gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer \
    -dNOPAUSE -dQUIET -dBATCH -dDetectDuplicateImages \
    -dCompressFonts=true -r400 -sOutputFile=$(T)-compressed.pdf 

T=autonomous\ survey

pdf:	$(T).tex
		$(PLT) $(T).tex
		$(PDFPLT) $(T).tex

$(T).dvi: $(T).tex
	$(PLT) $(T).tex
	$(XDV) $@&
	$(DPDF) $(T).dvi

p:	$(T).tex
	$(PLT) $(T).tex

b:	$(T).tex
	$(PLT) $(T).tex
	$(BTX) $(T)
	$(PLT) $(T).tex
	$(PDFPLT) $(T).tex

x:	$(T).dvi
	$(XDV) $(T).dvi&	

f:	$(T).dvi
	$(DPDF) $(T).dvi

s:	$(T).dvi
	$(DPS) $(T).dvi
	$(PS2PDF) $(T).ps
	rm $(T).ps

e:	$(T).tex
	$(EMCS) $(T).tex &

a:	$(T).pdf
	$(AC) $(T).pdf& 

zip:    $(T).pdf
	$(GS) $(T).pdf 

spell:
	aspell -t --dont-tex-check-comments -c $(T).tex

style:
	style-check.rb -v $(T).tex

clean:
	rm *.dvi *.aux *.log *.bbl *.blg

erase: 
	rm *.dvi *.aux *.log *.pdf *.bbl *.blg


